Exceptional points and near-extremal boundary response in rotating BTZ black holes

We investigate whether the coalescence of long-lived quasinormal modes enhances the boundary response of rotating BTZ black holes. Using exact scalar solutions with mixed Robin boundary conditions and the retarded boundary correlator, we compare frequency-domain resonances and time-domain signals at fixed source and operator normalizations. An exceptional point (EP) can be crossed by varying the spin alone in a suitably selected fixed theory. Along a distinct near-extremal path that tracks the co-rotating EP surface by tuning the scalar mass and boundary coupling, a taller, narrower resonance coexists with a weaker but longer-lasting double-pole impulse response. The frequency-domain enhancement persists away from the EP and is therefore not unique to mode coalescence. Thus, the EP determines the double-pole structure and Jordan relaxation, but does not by itself determine the response strength, which also depends on the physical path and excitation protocol.

==> figures/ep_diagnostic_workflow.tex <==
\begin{figure}[H]
 \centering
 \begin{tikzpicture}[
  node distance=7mm and 8mm,
  every node/.style={font=\footnotesize},
  flowstep/.style={draw,rectangle,rounded corners=1.5pt,align=center,
    text width=0.265\textwidth,minimum height=14mm,inner sep=3pt},
  check/.style={draw,rectangle,rounded corners=1.5pt,align=center,
    text width=0.37\textwidth,minimum height=15mm,inner sep=3pt},
  arrow/.style={-{Latex[length=2mm,width=1.3mm]},line width=0.55pt}
 ]
  \node[flowstep] (problem) {Exact radial problem\\
    ingoing at the horizon\\real Robin data};
  \node[flowstep,right=of problem] (candidate) {Algebraic candidate\\
    $\mathcal H=\partial_w\mathcal H=0$,\quad
    $\partial_w^2\mathcal H\neq0$};
  \node[flowstep,right=of candidate] (defect) {Geometric and topology tests\\
    $\dim\mathcal E_{\rm EP}=1$; Jordan chain;\\one-loop QNM sheet exchange};

  \node[check,below=9mm of candidate,xshift=-0.12\textwidth] (ep)
    {Second-order QNM EP\\
     algebraic multiplicity two; geometric multiplicity one};
  \node[check,right=of ep] (consequences)
    {Independent physical consequences\\
     second-order boundary pole; quadratic energy-resolvent law\\
     at fixed generator and norm};

  \draw[arrow] (problem) -- (candidate);
  \draw[arrow] (candidate) -- (defect);
  \draw[arrow] (defect.south) -- (ep.north east);
  \draw[arrow] (ep) -- (consequences);
 \end{tikzpicture}
 \caption{Diagnostic logic used in this paper.  A double zero of the scalar
 characteristic function establishes algebraic multiplicity two but is only
 an EP candidate until the one-dimensional QNM eigenspace is verified.  Sheet
 exchange and eigenfunction coalescence test the defect directly.  The
 boundary double pole and the energy-norm resolvent are consequences and
 cross-checks, not parts of the definition.}
 \label{fig:ep_diagnostic_workflow}
\end{figure}

